AGPNet -- Autonomous Grading Policy Network

In this work, we establish heuristics and learning strategies for the autonomous control of a dozer grading an uneven area studded with sand piles. We formalize the problem as a Markov Decision Process, design a simulation which demonstrates agent-environment interactions and finally compare our simulator to a real dozer prototype. We use methods from reinforcement learning, behavior cloning and contrastive learning to train a hybrid policy. Our trained agent, AGPNet, reaches human-level performance and outperforms current state-of-the-art machine learning methods for the autonomous grading task. In addition, our agent is capable of generalizing from random scenarios to unseen real world problems.

==> initial_image.tex <==



\begin{figure*}
 \centering
 \begin{subfigure}[t!]{0.8\textwidth}
     \includegraphics[width=\textwidth]{images/real_color_exp.png}
    %  \caption{Real RGB colormap}
     \label{fig:exp_real_color}
 \end{subfigure}
%  \hfill
 \begin{subfigure}[t!]{0.8\textwidth}
     \includegraphics[width=\textwidth]{images/real_heightmap_exp.png}
    %  \caption{Real Heightmap}
     \label{fig:exp_real_hmap}
 \end{subfigure}
 \begin{subfigure}[t!]{0.8\textwidth}
     \includegraphics[width=\textwidth]{images/simulated_heightmap_exp.png}
    %  \caption{Simulation Heightmap}z
     \label{fig:exp_sim_hmap}
 \end{subfigure}
    \caption{Comparison between a simulated environment and a real dozer before and after the grading action is preformed. top row is the rbg images captured by our experiment setup \ref{Real_world_comparison}. middle row is the, heigh-map. both top and middle observations are projected to world coordinates. bottom row is the same state, as it was generated by our simulator. \rc{add a-e and make larger individual images}. (a) state space for initial state. (b-e) states after actions taken in simulated environment and in real one. This figure depicts the resemblance in simulated and real height-maps in the grading task. }
    \label{fig:sim2real_all}
\end{figure*}

==> table_params.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}


% paramaters for bc training - 
\begin{table}[ht]
\centering
{%
\begin{tabular}{|c|c|}
\hline
learning rate         & 1.00E-05   \\ \hline
train batch size      & 120        \\ \hline
validation batch size & 40         \\ \hline
validation percentage & 5          \\ \hline
downsample factor     & 3          \\ \hline
gaussian factor       & 3          \\ \hline
number of episodes    & 150        \\ \hline
use\_cl               & True/False \\ \hline
\end{tabular}%
}
\caption{Parameters for training BC algorithms (use\_cl is True if training with CL and False otherwise)}
\label{tab:bc_params}
\end{table}



% parameters for training rl 
\begin{table}[ht]
\centering
{
\begin{tabular}{|c|c|}
\hline
learning rate        & 1.00E-03   \\ \hline
downsample factor    & 3          \\ \hline
gaussian factor      & 3          \\ \hline
loss update interval & 100        \\ \hline
minibatch size       & 50         \\ \hline
value loss coefficient    & 0.0001     \\ \hline
gamma                & 0.95       \\ \hline
bc loss coefficient  & 1000       \\ \hline
scenario type        & random     \\ \hline
$\lambda_t$      & 0.05       \\ \hline
$\lambda_h$      & 5          \\ \hline
$\lambda_v$      & 10         \\ \hline
$\lambda_d$      & 10         \\ \hline
$\lambda_f$      & 1         \\ \hline
use\_cl               & True/False \\ \hline
use\_bc               & True/False \\ \hline
use\_res              & True/False \\ \hline
\end{tabular}}
\caption{Parameters for training RL algorithms. use\_cl, use\_bc and use\_res are boolean parameters that indicate which training was performed. }
\label{tab:rl_params}
\end{table}
